Learning Disturbances Online for Risk-Aware Control: Risk-Aware Flight with Less Than One Minute of Data

Recent advances in safety-critical risk-aware control are predicated on apriori knowledge of the disturbances a system might face. This paper proposes a method to efficiently learn these disturbances online, in a risk-aware context. First, we introduce the concept of a Surface-at-Risk, a risk measure for stochastic processes that extends Value-at-Risk -- a commonly utilized risk measure in the risk-aware controls community. Second, we model the norm of the state discrepancy between the model and the true system evolution as a scalar-valued stochastic process and determine an upper bound to its Surface-at-Risk via Gaussian Process Regression. Third, we provide theoretical results on the accuracy of our fitted surface subject to mild assumptions that are verifiable with respect to the data sets collected during system operation. Finally, we experimentally verify our procedure by augmenting a drone's controller and highlight performance increases achieved via our risk-aware approach after collecting less than a minute of operating data.

==> experimental_validation.tex <==
Complex aerodynamics is challenging to model and can degrades flight performance when ignored (\cite{neuralfly,folkestad2022koopnet}). Flying in windy, near ground, and tether environment introduces unsteady and nonlinear effects that are computationally expensive to model and only valid near steady-state conditions. Our proposed model augmentation method address this issue without \textit{apriori} knowledge of the disturbances. Thus, we validated our safe risk-aware control using a custom hexacopter tracking prescribed trajectory in the presents of unknown tether weights, ground effect, and unknown winds. All flight tests are performed at Caltech's Center for Autonomous System and Technology arena equipped with an Optitrack motion capture system that samples and streams the rotor-craft pose at 190 Hz. A safeguard tether attaches to the hexacopter frame and a $\sim\!\!200\,$g passive weight eliminate slack which may also induce modeled disturbances. We desired a sufficiently challenging periodic flight path that exercises the controller to operate in the presents of ground effect and axial descent. Further, the Caltech Real Weather Wind Tunnel is employed to generate horizontal winds that are unknown to the system. 

Using the simplest reduce order for the hexacopter, the single integrator model for linear position, $\dot{\mathbold{x}} = \mathbold{v}$, where the linear velocity $\mathbold{v}$ is the control input. The commanded velocity input is then tracked by the onboard flight controller, a Hex Cube Orange running a PX4 autopilot \cite{px4}. With the risk-aware control augmentation, (discussion a little), we should the augmented controller significantly out performs the nominal controller. (Need to assert the benefit our statistical guarantees obtained from our method)


\begin{figure}[t]
    \centering
    \includegraphics[width = \textwidth ]{l4dc-2023/Figures/secondone.pdf}
    \vspace{-0.2 in}
    \caption{Experiment result, need to think of how to plot the improvement. Make be do one with just ground effect and one with groud effect + wind tunnel.}
    \vspace{-0.2 in}
    \label{fig:sar_examples}
\end{figure}




